Robust Offline Reinforcement learning with Heavy-Tailed Rewards

This paper endeavors to augment the robustness of offline reinforcement learning (RL) in scenarios laden with heavy-tailed rewards, a prevalent circumstance in real-world applications. We propose two algorithmic frameworks, ROAM and ROOM, for robust off-policy evaluation and offline policy optimization (OPO), respectively. Central to our frameworks is the strategic incorporation of the median-of-means method with offline RL, enabling straightforward uncertainty estimation for the value function estimator. This not only adheres to the principle of pessimism in OPO but also adeptly manages heavy-tailed rewards. Theoretical results and extensive experiments demonstrate that our two frameworks outperform existing methods on the logged dataset exhibits heavy-tailed reward distributions. The implementation of the proposal is available at https://github.com/Mamba413/ROOM.

==> Mis/packages.tex <==



% \usepackage[utf8]{inputenc}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{textcomp}
\usepackage{enumitem}
\usepackage{datetime2}
\usepackage{multirow}
\usepackage[font=small,labelfont=bf]{caption}
\doublespacing
\usepackage{xcolor}



% \usepackage{lineno}
% \linenumbers



% % provide the commands in case amssymb is not loaded
% \providecommand{\beth}{}
% \providecommand{\gimel}{}
% \providecommand{\daleth}{}
% % renew the commands
% \newcommand{\mathhebrew}[1]{\text{\cjhebfamily#1}}
% \renewcommand{\aleph}{\mathhebrew{\char'047}}
% \renewcommand{\beth}{\mathhebrew{\char'142}}
% \renewcommand{\gimel}{\mathhebrew{\char'147}}
% \renewcommand{\daleth}{\mathhebrew{\char'144}}

% \usepackage{unicode-math}
% \usepackage{libertine}
% \setmathfont[range={\beth,\gimel,\daleth,\aleph}]{Linux Libertine O}   

